A deep learning model for estimating story points

Although there has been substantial research in software analytics for effort estimation in traditional software projects, little work has been done for estimation in agile projects, especially estimating user stories or issues. Story points are the most common unit of measure used for estimating the effort involved in implementing a user story or resolving an issue. In this paper, we offer for the \emph{first} time a comprehensive dataset for story points-based estimation that contains 23,313 issues from 16 open source projects. We also propose a prediction model for estimating story points based on a novel combination of two powerful deep learning architectures: long short-term memory and recurrent highway network. Our prediction system is \emph{end-to-end} trainable from raw input data to prediction outcomes without any manual feature engineering. An empirical evaluation demonstrates that our approach consistently outperforms three common effort estimation baselines and two alternatives in both Mean Absolute Error and the Standardized Accuracy.

==> LSTM.tex <==
\section{Deep Learning of Text Features}
\label{section:LSTM}

We aimed to build a model which automatically transforms the title, description, and comments of an issue to  feature vectors that encodes their semantic meaning (i.e. text representation). Such pieces of text present a great challenge for feature extraction due to their complex linguistic structures hidden in sequence of characters. To aid discussion, we use an example of how the title of issue MESOS-3861 (``Authenticate quota requests") in the Apache Mesos project can be transformed into a real-valued vector.

The most popular text representation is Bag-of-Words (BoW) \cite{Sivic2003,Tirilly2008}, where a text is represented as a vector of word counts. For example, the title of issue MESOS-3861 would be converted into a sparse binary vector of  vocabulary size, whose elements are mostly zeros, except for those at the positions designated to ``authenticate", ``quota" and ``requests". The BoW representation, however, has several crucial drawbacks. Firstly, it is expensive to store and process, as the number of words is often of tens of thousands. Secondly, it effectively destroys the sequential nature of text. Finally, words do not necessarily capture the semantic structure of text. An alternative, which has gained popularity in software engineering, is using topic models such as Latent Dirichlet Allocation (LDA) \cite{Blei2012}. While LDA extracts thematic topics out of a text, it works directly on the BoW representation, and thus does not respect the sequential properties in text.

In this paper, we propose to use an alternative, novel feature extraction method that correctly models the sequential structure of text. The method is called Long Short-Term Memory (LSTM) which is based on Recurrent Neural Networks (RNN), a deep learning framework that has recently proved to be very powerful in many domains such as language models \cite{sundermeyer2012lstm}, speech recognition \cite{graves2013speech} and video analysis \cite{yue2015beyond}. The primary novelty (with respect to the traditional feature extraction) is that features are learned in an \emph{unsupervised} manner from \emph{raw characters} without any manual processing. We now briefly explain how LSTM works and describe how it is used for text representation.


%\subsection{Recurrent Neural Networks}
\subsection{Long Short-Term Memory}

The most powerful deep learning architecture at present is Neural Networks \cite{lecun2015deep}. A standard Neural Network is a mapping from input to output. For sequential data, a set of Neural Networks are sequentially connected to form a Recurrent Neural Network. While a feedforward neural network maps an input vector
into an output vector, an RNN maps a sequence into a sequence. Let
$\xb_{1},...,\xb_{n}$ be the input sequence and $y_{1},...,y_{n}$
be the sequence of corresponding labels. At time step $t$, the model
reads the input $\xb_{t}$ and the previous state $\hb_{t-1}$
to compute the state $\hb_{t}$. At each step, the hidden state $\hb_t$ is used to predict the output $y_t$.

Learning is usually by maximizing the likelihood of the output sequence given the input sequence:
\[
L\left(y_{1:n}\mid\xb_{1:n}\right)= \sum_{t=1}^{n}\log\left(y_{t}\mid\xb_{1:t}\right)
\]

%\subsection{Long-Short Term Memory}

While RNNs are theoretically powerful, they are difficult to train for long sequences. Long Short-Term Memory (LSTM) \cite{hochreiter1997long,gers2000learning} is a RNN variant that solves this problem. It achieves the effectiveness by several mechanisms.
The most important element is short-term memory -- a vector that stores accumulated experience over time.
The information stored in the memory is refeshed at each time step through partially forgetting old, irrelevant
information and accepting fresh new input. However, only some parts of the input will be added to the memory through
a selective input gate. Once the memory has been refreshed, an output state will be read from the memory through an output gate.
The output state $\hb_t$ is then used to predict the label. The reading of the new input, writing of the output,
and the forgetting are all learnable. The model training is identical to that of standard RNNs.

%Central to an LSTM is a linear self-loop
%memory cell which is gated to moderate the amount of information flow
%into or from the cell. Fig.\ref{fig:RNN_LSTM}(b) describes an LSTM
%unit. Instead of a simple RNN unit, an LSTM unit has a memory cell
%$\cb_{t}$ at time $t$. The information flowing through the memory
%cell is controlled by three gates: an input gate $\ib_{t}$, an forget
%gate $\fb_{t}$ and an output gate $\ob_{t}$.
%
%\begin{eqnarray}
%\ib_{t} & = & \sigma\left(W_{i}\xb_{t}+U_{i}\hb_{t-1}+\bb_{i}\right)\label{eq:input-gate}\\
%\fb_{t} & = & \sigma\left(W_{f}\xb_{t}+U_{f}\hb_{t-1}+\bb_{f}\right)\label{eq:foget-gate}\\
%\ob_{t} & = & \sigma\left(W_{o}\xb_{t}+U_{o}\hb_{t-1}+\bb_{o}\right)\label{eq:output-gate}
%\end{eqnarray}
%where $W_{\{i,f,o\}}$, $U_{\{i,f,o\}}$, $\bb_{\{i,f,o\}}$ are parameters
%and $\sigma$ is sigmoid function. These set the values of gates in
%the range $\left(0,1\right)$.
%
%At each time step, the input features are first computed by passing
%input $\xb_{t}$ and the previous hidden state $\hb_{t-1}$ through
%a tanh function. The memory cell is updated through partially forgetting
%the previous memory cell and reading the moderated input features.
%Then a hidden state $\hb_{t}$ is computed based on the memory $\cb_{t}$
%
%\begin{eqnarray}
%\gb_{t} & = & \mbox{tanh}\left(W_{c}\xb_{t}+U_{c}\hb_{t-1}+\bb_{c}\right)\label{eq:input-func}\\
%\cb_{t} & = & \fb_{t}*\cb_{t-1}+\ib_{t}*\gb_{t}\label{eq:mem-update}\\
%\hb_{t} & = & \ob_{t}*\mbox{tanh}\left(\cb_{t}\right)\label{eq:hidden-lsmt}
%\end{eqnarray}



\subsection{Feature learning for text}

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{LSTM-example.pdf}
	\caption{Word-based language model using LSTM for the text sequence ``Authenticate quota requests": words are
	first embedded into input vectors to be read into memory. The output state vectors are computed at each step
	to predict the next word. Finally, the sequence embedding vector is the mean of all output state vectors.}
	\label{figure:LSTM-example}
\end{figure}


This section presents our method for learning features from text using LSTM. Each of the three text components (description, title and comments) will be converted by the LSTM into a real vector of $m$  dimensions. Let us return to the running example, where the text is ``Authenticate quota requests". Our goal is to use LSTM to convert this sequence of words (and characters) into a vector of $m$ dimensions.

At this feature extraction stage, the story points are not used, and thus features will be learned in an unsupervised manner. Since there are no labels, we employ a technique popular in language modeling, that is at each step, we learn to predict the next word. This technique applied for RNNs has recently become popular, and it is now the state-of-the-arts in language modeling \cite{sundermeyer2012lstm,mikolov2010recurrent}. Let $w_{1},...,w_{n}$ be a sequence of words, we aim to estimate the probability of the next word given previous words. $P\left(w_{t}\mid w_{t-1},...,w_{1}\right)$ for $t=1,...n$. For example, our LSTM would estimate three probabilities: \emph{P(quota | Authenticate)}, \emph{P(requests | [Authenticate quota])} and \emph{P(<EOS> | [Authenticate quota requests])} where \emph{<EOS>} stands for ``end of sequence".

Figure \ref{figure:LSTM-example} shows how LSTM encodes the language model and converts the sequence into a real-valued vector. First, each word is embedded into a input vector of size $m_2$ through an embedding matrix. Second, the input vector is incorporated into the memory cells of the LSTM, from which an output state vector of size $m$ is emitted. This output vector is used to predict the next word in the sequence. Finally, the sequence embedding vector is the mean of all output vectors.

%In an RNN, the input sequence is $w_{1},...,w_{n-1}$ and the corressponding output sequence is $w_{1},...,w_{n}$.

However, a major bottleneck for this approach is the computation since the training time is proportional to vocabulary size. Thus for our work, we replace the words with the characters (including whitespace and special characters). For example, the first several conditional probabilities are: $P(u | A), P(t | [A u]), P(h | [A u t])$ and so on. While the word vocabulary is typically very large (ranging from tens to hundreds of thousands), and is usually growing with corpus size (words are not necessarily from real dictionary), the set of characters is small (70 for English \cite{Zhang2015}) and fixed. This leads to a huge boost in speed by several orders of magnitude. The character-based approach challenges the long-term view that words are the smallest semantic unit. However, latest evidences have demonstrated that characters are equally predictive in deep learning frameworks \cite{Zhang2015,kim2015character,gillick2015multilingual}.

Different from existing language work in NLP where each sentence is modelled as a sequence, our main interest is to model the entire document (e.g. the description or the comments of an issue), which consists of multiple sentences. Since our approach is character-based, a sentence boundary can be treated as a white-space character and the entire document is treated as a long sequence of characters. To the best of our knowledge, this treatment is novel.

Why will this approach work? There are several reasons. Firstly, thanks to the power of LSTMs -- it can deal with very long sequences (up to thousands of steps). Secondly, the regularities in text are captured in both the local context (sentences) and global context (document). The language model formulation dictates that the information accumulated thus far through LSTM memory is rich enough to predict the next character.

%Let $c_{1},...,c_{n}$ be a sequence of characters and symbols, including white spaces, the LSTM models
%the probability $P(c_{t}\mid c_{t-1},...,c_{1}).$ Each character
%$c_{t}$ in the sequence $c_{1},...,c_{n}$ is embedded into a distributed
%continuous vector $\xb_{t}$ using an embedding matrix $W\in\mathbb{R}^{|V|*m}$,
%where $|V|$ is the total number of unique characters
%
%\[
%\xb_{t}=W_{c_{t}}
%\]
%and then the input sequence $\xb_{1},...,\xb_{n-1}$ is fed to a LSTM
%network to predict the sequence of corressponding outputs $c_{1},...,c_{n}$.
%
%The embedding matrix $W$ and LSTM parameters are learned through
%Back Propagation Through Time algorithm \cite{werbos1990backpropagation}.
%
%After the learning phase, the feature vector of a sequence is computed.
%The input sequence $c_{1},...,c_{n-1}$ is passed to the LSTM to generate
%the sequence of hidden states $\hb_{1},...,\hb_{n-1}$. The feature
%vector $\ub$ is the mean of the hidden state vectors:
%\[ \ub=\frac{1}{n}\sum_{t=0}^{n-1}\hb_{t}\]

The character-based language model is learned in an unsupervised fashion (i.e., without story point labels). Once learned,
we just need to compute the output states $\hb_t$ and average them to derive the document-level embedding vector. In our study, titles, descriptions, and comments are learned separately. Each
title, description, or comment file is consider as a sequence of
character so each of them has a feature vector of $m$ dimensions.
Each data point would consist of three feature vectors: title, description,
and comment vectors. For a data point with more than one comment files,
its comment feature vector is the mean of the vectors of all comment
files. For data points without comment files, its comment feature
vector is set to be 0. In our study, we defined $m=100$ (i.e. 300 features for text representation) which is reasonable when compared compressing size of issue's textual data with LSTM running time. 


==> background.tex <==
\section{Background}\label{sect:background}
\subsection{Recurrent Neural Network} 

A Recurrent Neural Network (RNN) \cite{hochreiter2001gradient} is a simple single-hidden-layer neural network repeated multiple times. While a feedforward neural network maps an input vector into an output vector, an RNN maps a sequence into a sequence. Let $\wb_{1},...,\wb_{n}$ be the input sequence (e.g. words in a sentence) and $\yb_{1},...,y_{n}$ be the sequence of corresponding labels (e.g. the next words). At time step $t$, a standard RNN model reads the input $\wb_{t}$ and the previous hidden state $h_{t-1}$ to compute the hidden state $\hb_{t}$ as follows.

\begin{equation}\label{eq:hidden-state}
\hb_{t}=\sigma\left(\bb+W_{tran}\hb_{t-1}+W_{in}\wb_{t}\right)
\end{equation}
where $\sigma$ is a nonlinear element-wise transform function, and $\bb$, $W_{tran}$ and $W_{in}$
are parameters. The hidden state is used to produce an output at each step $t$. For example, the output of predicting the next word in a sentence would be a vector of probabilities across our vocabulary, i.e. $softmax(V\hb_{t})$.

An RNN shares the same parameters, i.e. ($W_{tran}$, $W_{in}$, $V$) , across all steps since essentially the same task (e.g. predicting the next word in a sentence) is performed at each step, just with different inputs. Hence, using an RNN significantly reduces the total number of parameters which we need to learn. The RNN model is trained using many input sequences with known actual output sequences (e.g. sentences in a text corpus). Learning is typically done by minimizing the error (i.e. the log-loss $L$) between the actual output and the predicted output by adjusting the model parameters. Learning involves computing the gradient of $L(\thetab)$ during the backpropagation phase, and parameters are updated using a stochastic gradient descent (SGD). It means that parameters are updated after seeing only a small random subset of sequences.

The critical problem with standard RNNs however lies here where the magnitude of weights in the transition matrix $W_{tran}$ (used in Equation~\ref{eq:hidden-state}) can have a strong effect on the learning process. This is because during the gradient backpropagation phase, the gradient signal can be multiplied a large number of times (as many as the number of code tokens in a sequence) by the transition matrix. If the weights in this matrix are small, it can result in the problem of \emph{vanishing gradients} where the gradient signal becomes so small that the learning gets very slow or even stopped. This makes standard RNNs not suitable for learning long-term dependencies. On the other hand, the large weights can lead to a large gradient signal (e.g. \emph{exploding gradient}), which can cause learning to diverge.


\subsection{Long Short-Term Memory}

Long Short-Term Memory (LSTM) \cite{hochreiter1997long,gers2000learning} is a special variant of RNN. It has a \emph{memory cell} $c_t$ (see Figure \ref{fig:LSTMunit}). This cell stores accumulated memory of the context, which is a mechanism to deal the vanish and exploding gradient problems. The amount of information flowing through the memory cell is controlled by three gates (an \emph{input gate}, a \emph{forget gate}, and an \emph{output gate}), each of which returns a value between 0 (i.e. complete blockage) and 1 (full passing through). All these gates are \emph{learnable}, i.e. being trained with the whole code corpus to maximize the predictive performance of the language model.

Let us now explain how an LSTM unit works. First, an LSTM unit decides how much information from the memory of previous context  (i.e. $c_{t-1}$) should be removed from the memory cell. This is controlled by the forget gate $\fb_{t}$, which looks at the the previous output state $h_{t-1}$ and the current code token $w_t$, and outputs a number between 0 and 1. A value of 1 indicates that all the past memory is preserved, while a value of 0 means ``completely forget everything''. In our example in Listing \ref{example}, the memory cell might keep information about the \texttt{writer} stream, so that it remembers this open stream needs closing later. When we see this stream being closed, we want to forget it.


%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.5\linewidth]{figs/LSTMcell}
%	\caption{The internal structure of an LSTM for code processing}
%	\label{fig:LSTMunit}
%\end{figure}

The next step is updating the memory with new information obtained from the current code token $w_t$. In a similar manner to the forget gate, the input gate $\ib_{t}$ is used to control which new information will be stored in the memory. For example, if $w_t$ is the new open stream, we want to add it into the memory cell so that we remember closing it later. Finally, information stored in the memory cell will be used to produce an output $h_t$. The output gate $\ob_t$ looks at the current code token $w_t$ and the previous hidden state $h_{t-1}$, and determines which parts of the memory should be output. For example, since it just saw the token \texttt{new}, it might want to output information relevant (e.g. constructor forms) to the initialization of the object declared previously, in case that what is coming next. It is important to note here that LSTM computes the current hidden state based on not just only the current input $w_t$ and the previous hidden state $h_{t-1}$ (as done in standard RNNs) but also the current memory cell state $c_t$, which is \emph{linear} with the previous memory $c_{t-1}$. This is the key feature allowing an LSTM model to learn long-term dependencies in text documents. 


==> feature.tex <==

\section{Story point datasets}
\label{section:datasets}

%In this section, we describe how data was collected and processed for our study and the features extracted from data. Since, effort estimation using story points in Agile is not only solely depended on a task complexity, but also experiences of teams. Thus, we extract not only features of an issue, but also features of participants who involved with an issue (i.e. reporter, assignee, and estimator). We have also propose a novel approach by applying Long-Short Term Memory (LSTM) technique on textual information of an issue (i.e. tile, description, and comments) to represent textual data as features to build story point estimators. These details will be discussed in this section.

A number of publicly available datasets (e.g. China, Desharnais, Finnish, Maxwell, and Miyazaki datasets in the PROMISE repository \todo{citehere}) have become valuable assets for many research in software effort estimation in the recent years. Those datasets however are only suitable for estimating efforts at the project level. To the best of our knowledge, there is currently no publicly available dataset for effort estimation at the issue level. Thus, we needed to build such a dataset for our study and made it publicly available (both raw data and in spreadsheet format) at \todo{XXX} for further research in this area.


\subsection{Data collecting and processing}

To collect data for our dataset, we looked for issues that were estimated with story points. JIRA\footnote{\url{https://www.atlassian.com/software/jira}} is one of the few widely-used issue tracking system that supports agile development (and thus story point estimation) with its JIRA Agile plugin. Hence, we selected six major open source ecosystems that uses the JIRA issue tracking system: Apache, Duraspace, Atlassian, Moodle, MuleSoft, and Spring. Apache\footnote{\url{https://issues.apache.org/jira/secure/Dashboard.jspa}} hosts a family of related projects sponsored by the Apache Software Foundation. The Atlassian\footnote{https://jira.atlassian.com/secure/Dashboard.jspa} repository has a number of projects which provides project management systems and collaborative tools. Moodle\footnote{\url{https://tracker.moodle.org/secure/Dashboard.jspa}} is an e-learning platform that allows everyone to join the community in several roles such as user, developer, tester, and QA.  MuleSoft\footnote{\url{https://www.mulesoft.org/jira/secure/Dashboard.jspa}} provides software development tools and platform collaboration tools such as Mule Studio and API designer. Spring\footnote{\url{https://spring.io/projects}} has a number projects supporting application development frameworks.

\begin{table}[h]
	\centering
	\caption{Collected data}
	\label{table:total_issue}
	\resizebox{3in}{!}{%
\begin{tabular}{@{}lccc@{}}
	\toprule
	\multicolumn{1}{c}{Repository}                                           & \# collected issues                                          & \# projects                                          & \# issues SP                                          \\ \midrule
	Apache                                                              & 11,614                                                        & 3                                                 & 1,632                                                  \\
	Duraspace                                                           & 7,258                                                         & 6                                                 & 753                                                    \\
	Atlassian                                                           & 15,139                                                        & 25                                                & 2,872                                                  \\
	Moodle                                                              & 7,631                                                         & 1                                                 & 974                                                    \\
	MuleSoft                                                            & 3,170                                                         & 31                                                & 2,956                                                  \\
	Spring                                                              & 12,106                                                        & 2                                                 & 3,722                                                  \\\midrule
	Total                                                               & 56,918                                                        & 68                                                & 12,909                                                 \\\bottomrule
	\multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}%ecos.: ecosystem name, \\ 
    %\# collected issues.: number of collected issues, \\ 
    \# projects: number of projects having issues with story points, \\ 
    \# issues SP: number of issues assigned with story points\end{tabular}} \\
\end{tabular}%
}
\end{table}

There are more than 100 projects hosted on Apache that use JIRA tracking system. We found that only three of them (Apache Mesos, Apache Usergrid, and Apache Aurora) uses JIRA Agile and have issues with story points. We then used the Representational State Transfer (REST) API\footnote{https://docs.atlassian.com/jira/REST/latest/} provided by JIRA to query and collected 11,614 issue reports between \emph{January 26, 2004} to \emph{January 12, 2016} from those three Apache projects. Similarly, we collected 7,258 issues between \emph{February 14, 2007} to \emph{January 12, 2016} from 6 projects in Duraspace. For the Atlassian repository, 15,139 issues opened from \emph{September 29, 2004} to \emph{January 12, 2016} were collected from their ecosystem. For Moodle, MuleSoft, and Spring, we collected issues opened from \emph{September 9, 2003} to \emph{January 12, 2016}. Table \ref{table:total_issue} reports the data that we have collected.

For each project that we collected, we then identified issues which were not assigned a story point and excluded them from our dataset. In total, our dataset has  12,909 issues with story points from 68 projects. Table \ref{table:dataset} summarizes the characteristics of the top ten projects (with respect to the number of issues with story points). Details of the remaining projects in our dataset can be found here \todo{url}

\todo{Make Table 2 into one column. Reduce font size to footnote size. Remove modeSP, varSP to save spaces}
\begin{table*}[ht]
	\centering
	\caption{The top ten projects (with respect number of issues in our dataset}
	\label{table:dataset}
	\resizebox{5.9in}{!}{%
		\begin{tabular}{@{}llcccccccc@{}}
			\toprule
			\multicolumn{1}{c}{ecos.} & \multicolumn{1}{c}{proj.} & \# issues SP & min SP               & max SP               & mean SP              & median SP            & mode SP              & var SP               & std SP               \\ \midrule
			Apache                    & Mesos                     & 1,000        & 1                    & 40                   & 3.28                 & 3                    & 3                    & 7.39                 & 2.71                 \\
			& Usergrid                  & 466          & 1                    & 8                    & 2.85                 & 3                    & 3                    & 1.94                 & 1.39                 \\
			Duraspace                 & DuraCloud                 & 610          & 1                    & 21                   & 2.17                 & 1                    & 1                    & 5.15                 & 2.26                 \\
			Atlassian                 & Bamboo                    & 521          & 1                    & 20                   & 2.42                 & 2                    & 1                    & 4.59                 & 2.15                 \\
			& Clover                    & 377          & 1                    & 53                   & 4.73                 & 2                    & 1                    & 49.89                & 4.06                 \\
			& Crucible                  & 330          & 1                    & 20                   & 3.14                 & 3                    & 1                    & 8.47                 & 2.91                 \\
			Moodle                    & Moodle                    & 974          & 1                    & 100                  & 15.1                 & 8                    & 5                    & 416.65               & 20.412               \\
			MuleSoft                  & Mule                      & 889          & 1                    & 21                   & 5.08                 & 5                    & 5                    & 12.24                & 3.5                  \\
			& Mule Studio               & 732          & 1                    & 34                   & 6.4                  & 5                    & 5                    & 29.01                & 5.39                 \\
			Spring                    & Spring XD                 & 3,508        & 1                    & 100                  & 3.85                 & 3                    & 1                    & 22.21                & 4.712                \\\midrule
			Total                     &                           & 9,407        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\\bottomrule
			\multicolumn{10}{c}{ecos.: ecosystem name, proj.: project name, \# issues SP: number of issues with story points}                                                                                                                     \\
		\end{tabular}%
	}
\end{table*}


%\begin{table*}[ht]
%	\centering
%	\caption{The top ten projects (with respect number of issues in our dataset}
%	\label{table:dataset}
%	\resizebox{5.9in}{!}{%
%		\begin{tabular}{@{}llcccccccc@{}}
%			\toprule
%			\multicolumn{1}{c}{ecos.} & \multicolumn{1}{c}{proj.} & \# issues SP & min SP               & max SP               & mean SP              & median SP            & mode SP              & var SP               & std SP               \\ \midrule
%			Apache                    & Mesos                     & 1,000        & 1                    & 40                   & 3.28                 & 3                    & 3                    & 7.39                 & 2.71                 \\
%			& Usergrid                  & 466          & 1                    & 8                    & 2.85                 & 3                    & 3                    & 1.94                 & 1.39                 \\
%			Duraspace                 & DuraCloud                 & 610          & 1                    & 21                   & 2.17                 & 1                    & 1                    & 5.15                 & 2.26                 \\
%			Atlassian                 & Bamboo                    & 521          & 1                    & 20                   & 2.42                 & 2                    & 1                    & 4.59                 & 2.15                 \\
%			& Clover                    & 377          & 1                    & 53                   & 4.73                 & 2                    & 1                    & 49.89                & 4.06                 \\
%			& Crucible                  & 330          & 1                    & 20                   & 3.14                 & 3                    & 1                    & 8.47                 & 2.91                 \\
%			Moodle                    & Moodle                    & 974          & 1                    & 100                  & 15.1                 & 8                    & 5                    & 416.65               & 20.412               \\
%			MuleSoft                  & Mule                      & 889          & 1                    & 21                   & 5.08                 & 5                    & 5                    & 12.24                & 3.5                  \\
%			& Mule Studio               & 732          & 1                    & 34                   & 6.4                  & 5                    & 5                    & 29.01                & 5.39                 \\
%			Spring                    & Spring XD                 & 3,508        & 1                    & 100                  & 3.85                 & 3                    & 1                    & 22.21                & 4.712                \\\midrule
%			Total                     &                           & 9,407        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\\bottomrule
%			\multicolumn{10}{c}{ecos.: ecosystem name, proj.: project name, \# issues SP: number of issues with story points}                                                                                                                     \\
%		\end{tabular}%
%	}
%\end{table*}


%Both the raw data is in JavaScript Object Notation (JSON) format and is available at XXX.


%To carry out the empirical study we collected the data of issues from six large open source ecosystems (i.e. issue tracking system) in which story points have been used in their effort estimation: Apache, Duraspace, Atlassian, Moodle, MuleSoft, Spring. Apache is a web server originally designed for Unix environments. There are more than three hundred core members and ten-thousand peripheral members contributing to Apache's projects \cite{Iqbal2014}. All issues in Apache were recorded in Apache's issue tracking system\footnote{\url{https://issues.apache.org/jira/secure/Dashboard.jspa}}. There are several projects in their ecosystem (e.g. Mesos, Usergrid, and Aurora). Duraspace\footnote{https://jira.duraspace.org/} supports the digital asset management that contains a number of projects in their ecosystem e.g. VIVO, Islandora, and DuraCloud. Atlassian\footnote{https://jira.atlassian.com/secure/Dashboard.jspa} provides a software development project supporting tool including (e.g.,) issue track system, version control system, and document collaboration system. There are a number of projects (e.g. JIRA, Bamboo, and Clover) are contained in their ecosystem. Moodle is an e-learning platform that allows everyone to join the community in several roles such as user, developer, tester, and QA. The Moodle tracker\footnote{\url{https://tracker.moodle.org/secure/Dashboard.jspa}} is their ecosystem system which is used to collect issues and working items, and keep track issues status in development activities. MuleSoft\footnote{\url{https://www.mulesoft.org/jira/secure/Dashboard.jspa}} provides software development tools and platform collaboration tools such as Mule Studio and API designer. Spring\footnote{\url{https://spring.io/projects}} is an application development framework and it has approximately one-hundred contributors.

%All the six ecosystems use JIRA, a well-known issues and project tracking software that allows teams to plan, collaborate, monitor, and organize issues including assigning story points to issues following the agile methodology. We use the Representational State Transfer (REST) API\footnote{https://docs.atlassian.com/jira/REST/latest/} provided by JIRA to query and collected issue reports in JavaScript Object Notation (JSON) format.

%We collected a large number of issues from all six ecosystems which contain a number of projects (See Table \ref{table:total_issue}). For Apache, 11,614 issues opened from \emph{January 26, 2004} to \emph{January 12, 2016} were collected which consist of three projects with story points. We collected 7,258 issues from the Duraspace's ecosystem opened from \emph{February 14, 2007} to \emph{January 12, 2016} and found 6 projects with story points. For Atlassian, 15,139 issues opened from \emph{September 29, 2004} to \emph{January 12, 2016} were collected from their ecosystem. For Moodle, MuleSoft, and Spring, we collected issues opened from \emph{September 9, 2003} to \emph{January 12, 2016}. In total, we collected 56,918 issues (12,909 issues from 38 projects have story points).

%Since, we found that story points are not available in all issues and projects (i.e. some issues have not been assigned a story point) because effort estimation using story points could be recently applied by teams. Thus, story points have not been assigned to those prior issues (historical issues and projects). Moreover, some projects also have a small number of issues with story points. Including those issues in our dataset could affects our study. In our study, we thus selected only the projects that have issues with story points greater than three-hundred issues as it is reasonable and large enough for our study. However, our feature extraction exploited all collected issues e.g., all collected issues are took into account in order to determine the number of issues resolved by an assignee. We also carefully eliminated the demonstration projects from Atlassian ecosystem since those projects have been provided for testing their JIRA system.



T%able \ref{table:dataset} shows the number of collected issues, the number of issues with story points of each selected projects, and some statistical measures on story points (SP) from all projects. There are 10 projects from the six ecosystem have been included in our study. As can be seen that, teams tend to assign a low story point to issues. We thus carefully employed measures to evaluate the predictive performance of our approach as some measures bias towards underestimations (e.g., MRE) \cite{Sarro}. We also noted that the variance of story points in Moodle is high since 5\% of issues have been assigned story points of 100. \todo{url for download}



%\todo{do we need to explain about data availability? to show that our features is not fishing. or just mention in feature list}
%\todo{common features not specific to jira}
%\todo{not feature fishing}

\subsection{Issue's features}

Our dataset has a number of features describing an issue itself. Since we want to extract only features that exist across all the projects in our dataset, we choose standard, mandatory fields of a JIRA issue. To avoid leaking, the value of those features were extracted just before the time when a story point was assigned to the features. By analyzing the change log of an issue, we were able to reveal various information about the issue's history such as when a story point was assigned to an issue or when the description of an issue is changed.



%We extracted a number of features to characterize an issue. These features are indicators which are then used to estimate story points. Generally, teams perform story point estimation before resolving issues (e.g. planning for iterations). In our study, teams spent 33 days after issue creation time to estimate story points (average across all projects). However, there are 61\% of issues in our dataset have been assigned a story point at issue creation time. The features have been extracted respect to the story point assign time of an issue. Specifically, we consider only information available at the story point assign time of an issue (e.g. mandatory field). We initially extracted a broad range of features related to an effort, and then used feature selection techniques (see Section \ref{section:feature_selection}) to remove weak and redundant features. We now describe each of those features in detail.

\subsubsection{Type}

Each issue will be assigned a type (e.g. Task, Bug, New feature, Improvement, and Documentation) which indicates the nature of the task associated with resolving the issue (e.g. fixing a bug or implementing a new feature). Each of those issue types require different efforts (e.g. implementing new features would requires more efforts than fixing bugs). Table \ref{table:stat_type} shows the top three of issue's type having the highest and lowest mean of story points (average across all projects).
We note that the issue types are defined specifically in each of the five selected projects. For example, while there is no ``Document'' type for issues in the Moodle project, this type exists in the issues of Duraspace.

\begin{table}[h]
	\centering
	\caption{The highest/lowest mean of story points based on issue's types}
	\label{table:stat_type}
	\resizebox{2.9in}{!}{%
		\begin{tabular}{@{}lclc@{}}
			\toprule
			\multicolumn{1}{c}{Type} & mean SP & \multicolumn{1}{c}{Type} & mean SP \\ \midrule
			Epic                     & 23.63         & UX Story           & 2.15         \\
			New feature          & 9.97         & Third-party issue                 & 2          \\
			Sub-task                     & 8.88         & Technical Story                 & 1.71          \\ \bottomrule
		\end{tabular}%
	}
\end{table}

\subsubsection{Priority}

The issue's priority presents the order in which an issue should be attended with respect to other issues which effects directly to contributed efforts. For example, issues with blocker priority should be more concerned than issues with major or minor priority. Blocker priority is an issue that blocking other issues to be completed. As can be seen from Table \ref{table:stat_priority}, issues having \emph{Blocker} and \emph{Critical} as their priority have high story points, while issues having \emph{Trivial} as their priority was estimated as minimum efforts. Note that \emph{To be reviewed} priority are used in MuleSoft's projects as to indicate new features that required discussions.

\begin{table}[h]
	\centering
	\caption{The highest/lowest mean of story points based on priority (average across all projects)}
	\label{table:stat_priority}
	\resizebox{2.5in}{!}{%
		\begin{tabular}{@{}lclc@{}}
			\toprule
			\multicolumn{1}{c}{Priority} & mean SP & \multicolumn{1}{c}{Priority} & mean SP \\ \midrule
			Blocker                     & 7.21         & Major           	& 4.96          \\
			Critical          			& 6.51         & Minor   			 & 4.66          \\
			To be reviewed             	& 6.22         & Trivial            & 2.47          \\ \bottomrule
		\end{tabular}%
	}
\end{table}

%\subsubsection{Complexity of description} -- textual info. has been emploied by LSTM this is redundancy
\subsubsection{Changing of priority}

The changing of an issue's priority may indicate the shifting of its complexity which potentially affects an estimated effort. In our context, we are particularly interested in the number of times an issue's priority was changed which may affects to an effort estimation.
%For example, Valdivia et al. \cite{Garcia2014b} use the changing of priority as a feature to predict blocking bug.

\subsubsection{Number of subtasks}

A task (i.e. issue) can be decomposed into a number of subtasks. A high number of subtasks is required more efforts. For example, issue ID \emph{MULE-9109} in the Mulesoft project consisted of eleven sub-tasks and its estimated story point is 21.

\subsubsection{Number of issue links}

Issue linking allows teams to create an association between issues. There are several type of issue links (e.g. relates to, duplicate, and block). A resolving of an issue with a number of issue links requires more efforts, since developers should consider all linked issues (e.g. code conflict). For example, the story point of 13 has been assigned to issue ID \emph{MULE-7588} in the Mulesoft project which has 12 issue links.

\subsubsection{Number of issues that are blocked by this issue}

This feature is the number of issues that are blocked by this issue. Blocker is one of the issue linking types. This type of issue dependency indicates the complexity of resolving issues since it directly affects the progress of other issues (i.e. a blocked issue can not be resolved before a blocker issue). We thus deal with the blocker relationship separately.

\subsubsection{Number of issues that block this issue}

This feature is the number of other issues that are blocking this issue from being completed. Thus, the number of blocker issues indicates the complexity to solve an issue \cite{Garcia2014b}.

\subsubsection{Number of affect versions}

The ``Affect Version'' field of an issue specifies versions in which it has been found. One issue can be found in many versions. More effort is needed to resolve an issue with a high number of affected versions. For example, the story point of 40 has been assigned to issue \emph{MDL-38732} in the Moodle project since it affects to eight versions.

\subsubsection{Number of fix versions}

The ``Fix Version'' field on each issue indicates the release version(s) for which the issue was (or will be) fixed. Issues with a high number of fix versions need more effort in terms of developing, testing, and integrating (e.g. An intensive reviewing process is also required to validate that the resolving of an issue does not cause new problems for each fix version). For example, issue \emph{MDL-42767} in the Moodle project is targeted to be fixed in five versions which it has been assigned the story point of 13.


\subsubsection{Number of related components}

This feature is a number of components related to an issue. An issues with a high number of related components indicate a high complexity.

\subsubsection{Changing of description}

This feature is the number of times in which the issue's description was changed. The description of an issue is important to all stakeholders of the issue. Changing the description of an issue can indicates the complexity of an issue which shows that issue is not stable and may also create confusion and misunderstanding. From our investigation, 49\% of issues having more than five times in changing of description has a potential to obtain the story point higher than 8.

\subsection{Features of participants}

Effort estimation is not only a matter of complexity of a task \cite{Usman2014a}. Teams usually take the members who involved with an issue into an account (e.g. skill and experience). Especially, in story point estimation, teams usually estimate less effort (i.e. lower story points) on issues that teams or developers are familiar with.
Thus, we attempt to characterize team members who involved with an issue using these features. The features of participants cover three different roles: a reporter, an assignee (i.e. a developer), and an estimator. A reporter is a person who create (i.e. report) an issue. An assignee is the one who has been assigned to resolve an issue. A story point of an issue is assigned by an estimator. Note that, there are 31.25\% of issues have the same user as reporter, assignee, and estimator (e.g. issue \emph{MESOS-3213} in the MESOS project). However, each feature is extracted separately.
%\todo{The intuition is the more they work the less sp, since they familiar with the task}

\subsubsection{Reporter reputation}

Reporter reputation has been studied in previous work in mining bug reports (e.g. \cite{Bhattacharya2011a,Hooimeijer2007a,Zimmermann2012a}). For example, Zimmermann et. al. \cite{Zimmermann2012a} found that bugs reported by low reputation people are less likely to be reopened. Hooimeijer et al. \cite{Hooimeijer2007a} used bug opener's reputation to predict whether a new bug report will receive immediate attention or not. Choetkiertikul et al. \cite{Morakot2015} used issue reporter's reputation to predict a risk of delayed issues. In our context, reporter reputation could indicates an issue's complexity (i.e. an issue reported by high reputation reporter may important to a project which may requires higher effort to resolve). We use Hooimeijer's submitter reputation \cite{Hooimeijer2007a} as follows:

\[  reputation(D) = \frac{\left | opened(D) \cap fixed(D) \right |}{\left | opened(D) \right |+1} \]

The reputation of a reporter $D$ is measured as the ratio of the number of issues that $D$ has reported and resolved to the number of issues that $D$ has reported plus one.

%\subsubsection{Number of issues tested, reviewed, and resolved by a reporter, an assignee, and an estimator}
\subsubsection{Number of issues tested, reviewed, and resolved by a reporter}

We extracted three features regarding a reporter: number of issues tested by a reporter, number of issues reviewed by a reporter, and number of resolved by reporter. The previous feature (reporter reputation) only considers the number of issues opened and resolved by a reporter, while these features regarding a reporter indicate how a reporter involve in a project.

%\subsubsection{Number of comments made by a reporter }

\subsubsection{Number of issues tested, reviewed, and resolved by an assignee}

There are also three extracted features regarding an assignee: number of issues tested by an assignee, number of issues reviewed by an assignee, and number of resolved an assignee. An assignee is assigned to resolve an issue. These three features indicate experiences of an assignee in terms of testing, reviewing, and resolving tasks which could affect to effort estimation. For example, a story point of a test-related issue has been assigned to an assignee who used to test a number of issues would be less than assigned to others with no experience in testing.

It could be however noted that an assignee is not always available at story point assign time (i.e. an assignee has been assigned after assigning a story point). We thus treated it as a missing data in order to distinct between zero (e.g. have not resolved any issues) and not being assign an assignee.
% We discuss how we handle the problem of missing data in Section \todo{ref missing data technique}.

%\subsubsection{Number of comments made by an assignee}

\subsubsection{Number of issues tested, reviewed, and resolved by an estimator}

Usually, team members must involve in story point estimation. An estimator however is the one who make a final decision and assign a story point to an issue. Thus, we also extracted three features regarding an estimator: number of issues tested by an estimator, number of issues reviewed by an estimator, and number of resolved an estimator. Note that an estimator is not explicitly recorded as an issue attribute (reporter and assignee can be extracted directly from an issue record). An estimator is identified from issue change log by extracting a user who assigned a story point.

Note that the features of participants are extracted regarding the story point assign time of an issue e.g., the number of issues resolved by assignee of one assignee may be not the same in two different issues. We need to be more realistic and prevent the problem of information leakage \cite{Kaufman2011}.

% We exploited all collected issues in the features extraction not only issues that have been assigned a story point. Those issues must be counted toward the features.

%\subsubsection{Number of comments made by an estimator}

%\subsubsection{Number of issues resolved by an assignee}

%\subsubsection{Number of issues resolved by an estimator}

%\subsubsection{Number of issues reviewed by a reporter, an assignee, and an estimator}

%\subsubsection{Number of issues reviewed by an assignee}

%\subsubsection{Number of issues reviewed by an estimator}

%\subsubsection{Number of issues tested by a reporter, an assignee, and an estimator}

%\subsubsection{Number of comments made by a reporter, an assignee, and an estimator} commenct is used by LSTM



%We must also note that all extracted features are extracted according to story point estimation time (i.e. prediction time), for example number of comments made by reporter before story point estimation time. In our study, we design to consider only information available before estimation time in order to prevent the problem of information leakage \todo{cite}.

\subsection{Long-Short Term Memory}
\todo{describe LSTM} 

==> model.tex <==
\section{Feature Selection}
\label{section:feature_selection}

Simplification of models (i.e. Sparse models) --  those with a small number of features --
are desirable since they are easier to interpret and acted upon by model users. They are also critical to enhanced generalization by reducing over-fitting when training data is limited compared to the number of possible attributes. In our case, textual features can be large. Hence, we employ \emph{Least Absolute Shrinkage and Selection Operator (LASSO)} \cite{Shrinkage1996} to select a compact subset of features that provide a good predictive performance \cite{Guyon2003}.

LASSO is a regression analysis method that performs both feature selection and regularization in order to enhance the prediction accuracy by  penalizing the magnitude of the regression coefficients. Specifically, given a set of features $x_1, x_2, x_3, ... , x_p$ and an outcome  (i.e. story point) $y$, the LASSO fits a linear model:

\[ \hat{y} = b_{0} + b_{1}x_{1} + b_2x_2 + ... + b_px_p \]

The objective of lasso is to solve:

%\[ min\left \{ \frac{1}{N} \sum_{i=1}^{N}(y_i - \hat{y})^2 \right \} subject\ to \sum_{j=1}^{p}\left | b_j \right | \leq s \]

\[ min\left \{  \sum_{i=1}^{N}(y_i - \hat{y_i})^2 \right \} subject\ to \sum_{j=1}^{p}\left | b_j \right | \leq s \]

where $s$ is a prespecified free parameter that determines the amount of regularization  and ${b_j}$ are regression coefficients. A smaller s will drive more coefficients towards zeros, effectively removing the effect of those features. We then remove features zero coefficients $\beta_j$.

\section{Story Point Estimation Models}
\label{section:estimation-models}

%Our estimation models are then built from the selected features of issues and participants (using \emph{LASSO}) and the features from LSTM. We employ state-of-the-art randomized ensemble methods: Random Forests (RF) to train our story point estimation models. RF was the best performing modeler and have frequently won recent data science competitions (e.g. Kaggle\footnote{https://www.kaggle.com}). However, there are a number of benchmarks and state-of-the-art techniques for effort estimations. In our study, we also employ three widely-used and well-studied state-of-the-art effort estimation methods: Automatically Transformed Linear Model (ATLM) \cite{Whigham2015}, Case-Based Reasoning (CBR) \cite{Shepperd1997}, and Classification and Regression Trees (CART) \cite{L.BreimanJ.H.FriedmanR.A.Olshen1984} to compare with our proposed approach. Moreover, as recently suggested by Sarro et al. \cite{Sarro} that a good effort estimation model should outperform with baseline estimators: Random Guessing, Mean/Median Effort. This section briefly describes these methods.

Using the issues in our dataset, we were able to build and train a number of estimation models. These models take as input a set of predictors (or the features we selected such as priority, type and so on), and returns a scalar value representing the story points estimated for an issue having the characteristics captured by the predictors. Different prediction approaches use the predictors in different ways. The estimation models built in our study are based on four widely-used and well-studies state-of-the-art software effort estimation methods which are described as follows.

%, namely Automatically Transformed Linear Model (ATLM) \cite{Whigham2015}, Case-Based Reasoning (CBR) \cite{Shepperd1997}, Classification and Regression Trees (CART) \cite{L.BreimanJ.H.FriedmanR.A.Olshen1984}, and the randomized ensemble method Random Forests (RF).


\textbf{Linear Regression.} We used the Automatically Transformed Linear Model (ATLM) \cite{Whigham2015} recently proposed as the baseline model for software effort estimation. Although ATLM is simple and requires no parameter tuning, it performs well over a range of various project types in the traditional effort estimation \cite{Whigham2015}.

\textbf{Case-Based Reasoning (CBR).} CBR has been successfully used in estimating the development effort of a software project \cite{Shepperd2003}. Thus, we also built a CBR model for story point estimation. In order to estimate story points for a new issue (i.e. target issue) which is characterized by its set of features, we retrieve issues in the past that are relevant to this issue. In order to do so, we use a similarity function that measures the distance between the target issue and the other issues based on the values of these issues' features. We then used the mean story points of the $k$ most similar issues as the estimate for the new issue. Our CBR model uses the Euclidean distance measure between vector. We chose $k = 3$ since this setting produced the best performance in traditional effort estimation for projects as reported in \cite{Sarro}. In our work, CBR predictions are obtained using  \emph{knnsearch}\footnote{\url{http://au.mathworks.com/help/stats/knnsearch.html}} provided in Matlab.

% \cite{Quinlan1993}

\textbf{Classification and Regression Trees (CART).} CART is a classical machine learning method for effort estimation in software projects. CART is a decision tree in which decision nodes are generated based on the information gain using the value of each feature. Thus, CART offers an explainable model, which is one of the main advantages of this approach. Dependent variables in a classification tree takes a finite set of values, while those in a regression tree take continuous values (e.g. story points). We generated regression trees were using \emph{fitrtree}\footnote{\url{http://au.mathworks.com/help/stats/fitrtree.html}} provided in Matlab. The problem of overfitting easily occurs in CART. We thus also apply the pruning function ($level = 5$) and control the minimum number of leaf node observations ($MinLeafSize = 5$). 

\textbf{Random Forests (RF).} Ensemble methods refer to the use of many classifiers to make prediction \cite{Breiman2001a}. Previous research (e.g. \cite{Kocaguneli2012}) have demonstrated the effectiveness of ensemble methods in software effort estimation. RF \cite{Breiman2001a} is an ensemble of decision trees. RF is a significant improvements of the decision tree approach by generating many classification and regression trees, each of which is built on a random resampling of the data, with random subset of variables at each node split. Tree predictions are then aggregated through voting. Since we deal with continuous values, regression trees are fitted instead of classification trees. In our work, we trained 100 regression trees using the \emph{randomeforest-matlab}\footnote{\url{https://code.google.com/archive/p/randomforest-matlab/}} package for Matlab.

%\todo{more about RF implementation and settings}.

%Previous research, \cite{Lessmann2008,Kamei2010} has shown that RF is one of the best for a wide range of problems. %In our work, we used Random Forests package for Matlab.

We would also like to perform a sanity check to see if the above statistical and machine learning models perform better than a number of baseline estimator. Thus, we implemented three simple estimation models as follows.

\textbf{Random Guessing} Random guessing is a naive benchmark used to assess if an estimation model is useful \cite{Shepperd2012}. In our context, it randomly assigns the story point value of another issue to the target issue. More precisely, it performs random sampling (with equal probability) over the set of issues with known story points, chooses randomly one issue from the sample, and uses the story point value of that issue as the estimate of the target issue. Random guessing does not use any information associated with the target issue, thus any useful estimation models should outperform random guessing.

\textbf{Mean/Median Effort} These methods are commonly used as baseline benchmarks for effort estimation. They use the mean or median story points of the past issues to estimate the target issue. 
